Debiasing Pre-trained Contextualised Embeddings

In comparison to the numerous debiasing methods proposed for the static non-contextualised word embeddings, the discriminative biases in contextualised embeddings have received relatively little attention. We propose a fine-tuning method that can be applied at token- or sentence-levels to debias pre-trained contextualised embeddings. Our proposed method can be applied to any pre-trained contextualised embedding model, without requiring to retrain those models. Using gender bias as an illustrative example, we then conduct a systematic study using several state-of-the-art (SoTA) contextualised representations on multiple benchmark datasets to evaluate the level of biases encoded in different contextualised embeddings before and after debiasing using the proposed method. We find that applying token-level debiasing for all tokens and across all layers of a contextualised embedding model produces the best performance. Interestingly, we observe that there is a trade-off between creating an accurate vs. unbiased contextualised embedding model, and different contextualised embedding models respond differently to this trade-off.

==> related-work_original.tex <==
\section{Related Work}
\label{sec:related}

Prior work on debiasing word embeddings can be broadly categorised into two groups depending on whether they consider static (\autoref{sec:static}) or contextualised word embeddings (\autoref{sec:context}). 
In this paper, we focus purely on debiasing contextualised word embeddings. 
However, for the completeness of discussion, we describe both categories of prior work. 

\subsection{Bias in Static Word Embeddings}
\label{sec:static}

In their pioneering work, \newcite{Tolga:NIPS:2016} proposed a post-processing approach that projects gender-neutral words into a subspace, which is orthogonal to the gender direction defined by a list of gender-definitional words.
They refer to words associated with gender (e.g., \emph{she}, \emph{actor}) as gender-definitional, and the remainder as gender-neutral.
They proposed a \emph{hard-debiasing} method where the gender direction is computed as the vector difference between the embeddings of the corresponding gender-definitional words, and a \emph{soft-debiasing} method, which balances the objective of preserving the inner-products between the original word embeddings, while projecting the word embeddings into a subspace orthogonal to the gender definitional words. 
%They use a list of gender-definitional words to train a support vector machine classifier, and use it to expand the initial set of gender-definitional words.
Both hard and soft debiasing methods ignore gender-definitional words during the subsequent debiasing process, and focus only on words that are \emph{not} predicted as gender-definitional by the classifier. 
Therefore, if the classifier erroneously predicts a stereotypical word as gender-definitional, it would not get debiased.

\newcite{Zhao:2018ab} modified the original GloVe~\cite{Glove} objective to learn gender-neutral word embeddings (GN-GloVe) from a given corpus.
They maximise the squared $\ell_{2}$ distance between gender-related sub-vectors, while simultaneously minimising the GloVe objective.
Unlike the above-mentioned methods, \newcite{kaneko-bollegala-2019-gender} proposed GP-GloVe, a post-processing method to preserve gender-related information, while removing discriminatory biases from stereotypical cases.
However, all prior debiasing methods require us to pre-define the biases in the form of explicit word lists containing gender and stereotypical word associations.

Adversarial learning methods~\cite{Xie:NIPS:2017,Elazar:EMNLP:2018,Li:2018ab} for debiasing first encode the inputs and then two classifiers are jointly trained -- one predicting the target task (for which we must ensure high prediction accuracy) and the other for protected attributes (that must not be easily predictable). 
However,  \newcite{Elazar:EMNLP:2018} showed that although it is possible to obtain chance-level development-set accuracy for the protected attributes during training, a post-hoc classifier trained on the encoded inputs can still manage to reach substantially high accuracies for the protected attributes. 
They conclude that adversarial learning alone does not guarantee invariant representations for the protected attributes.
\newcite{Ravfogel:2020} found that iteratively projecting word embeddings to the null space of the gender direction to further improve the debiasing performance. 

% WEAT, WAT, SemBias, WinoBias, OntoNotes (one para)
Several benchmark datasets have been developed for evaluating different types of word-level biases in static word embeddings.
Word Embedding Association Test~\cite[WEAT;][]{Caliskan2017SemanticsDA} quantifies various biases (e.g. gender, race and age) using semantic similarities between word embeddings.
It compares two same size sets of \emph{target} words (e.g. European and African names), with two sets of \emph{attribute} words (e.g. \emph{pleasant} vs. \emph{unpleasant}) using cosine similarity between the corresponding word embeddings to compute a normalised measure.
Word Association Test (WAT) is a method to measure gender bias over a large set of words~\cite{du-etal-2019-exploring}.
It calculates the gender information vector for each word in a word association graph created in the Small World of Words project~\cite[SWOWEN;][]{Deyne2019TheW} by propagating information related to masculine and feminine words using a random walk approach~\cite{Zhou2003LearningWL}.
SemBias dataset~\cite{Zhao:2018ab} contains three types of word-pairs: 
(a) \textbf{Definition}, a gender-definition word pair (e.g. hero -- heroine), 
(b) \textbf{Stereotype}, a gender-stereotype word pair (e.g., manager -- secretary) 
and (c) \textbf{None}, two other word-pairs with similar meanings unrelated to gender (e.g., jazz -- blues, pencil -- pen). 
It uses the cosine similarity between the gender directional vector, $(\vv{he} - \vv{she})$, and the offset vector $(\vec{a} - \vec{b})$ for each word pair, $(a,b)$, in each set to measure gender bias.

The ability to predict gender pronouns with equal probabilities for gender neutral nouns such as occupations has been used as a test for the gender bias in embeddings. 
WinoBias dataset contains two types of sentences that require linking gendered pronouns to either male or female stereotypical occupations.
In \textbf{Type 1}, co-reference decisions must be made using world knowledge about some given circumstances. 
However, in \textbf{Type 2}, these tests can be resolved using syntactic information and understanding of the pronoun.
It involves two conditions: the pro-stereotyped (\textbf{pro}) condition links pronouns to occupations dominated by the gender of the pronoun, and the anti-stereotyped (\textbf{anti}) condition links pronouns to occupations not dominated by the gender of the pronoun.
For a correctly debiased set of word embeddings, the difference between \textbf{pro} and \textbf{anti} is expected to be small. 

\subsection{Bias in Contextualised Word Embeddings}
\label{sec:context}

\newcite{may-etal-2019-measuring} extended WEAT using templates to create a sentence-level benchmark for evaluating bias called SEAT. In addition to the attributes proposed in WEAT, this paper proposes two additional bias types: angry black woman and double binds (when a woman is doing a role that is typically done by a man that woman is seen as arrogant). Tests show that modern sentence embeddings such as BERT, GPT and ELMo are less biased.
However, similar to WEAT, SEAT also only has positive predictive ability and cannot detect the absence of bias.
%On the other hand, the dictionary-based evaluation we conduct in this paper can be seen as a test for the absence of bias and complements the evaluations conducted using SEAT.

\newcite{bommasani-etal-2020-interpreting} evaluated the bias in contextualised embeddings by first distilling static embeddings from contextualised embeddings and then using WEAT tests for different types of biases such as gender (male, female)  racial (white, Hispanic, Asian) and religion (Christianity, Islam). They found that aggregating the contextualised embedding of a particular word in different contexts via averaging to be the best method for creating a static embedding from a contextualised embedding.

\newcite{Zhao:2019a} showed that contextualised ELMo embeddings  also learns gender biases present in the training corpus. 
Moreover, these biases propagate to a downstream coreference resolution task as well. 
They also showed that data augmentation by swapping gender helps more than neutralisation by projection. 
However, data augmentation requires re-training of the embeddings, which is often costly and we would like to avoid in this paper.

\newcite{kurita-etal-2019-measuring} created masked templates such as ``\_\_ is a nurse'' and used BERT to predict the masked gender pronouns. They proposed the log-odds between male and female pronoun predictions as a measure for evaluating gender bias in contextualised language models. 
Their experiments show that this bias measure to correlate well with human annotated bias datasets, and that BERT is biased according to this measure.
\newcite{karve-etal-2019-conceptor} learnt conceptor matrices using class definitions in the WEAT dataset and used the negated conceptors to  debias ELMo and BERT embeddings. 
They found that conceptor debiasing outperforms hard debiasing for ELMo embeddings,
but reported mixed results for BERT embeddings.

\newcite{dev2020on-measuring} proposed natural language inference as a method for evaluating the biases in embeddings.
Specifically, the goal is to ascertain if one sentence (i.e. premise) entails or contradictions another (i.e. hypothesis), or if neither conclusions hold (i.e. neutral).
The premise and hypothesis pairs are constructed in a manner to elicit various types of discriminative biases.
They showed that orthogonal projection to gender direction as proposed by  \newcite{DBLP:conf/aistats/DevP19} can be used to debias contextualised embeddings as well.
However, their method can be applied only to the noncontextualised layers (ELMo's Layer 1 and BERT's subtoken layer).
In contrast, our proposed method can be applied to \emph{all} layers in a pre-trained contextualised embedding and outperforms their method on the same natural language inference task.

%DB: 以下はあまりdebiasing関係ない．単にBERTでcoreferenceができるというだけの論文．書かなくて良い．
%Fine-tuning BERT has been an effective strategy for resolving gender ambiguous pronouns (GAP)~\cite{webster-etal-2019-gendered} in prior work, indicating that BERT already encoding much information related to grammatical gender~\cite{alfaro-etal-2019-bert}.
%BERT has shown to be able to reinstate masked gender pronouns in English coreference tasks~\cite{alfaro-etal-2019-bert,chada-2019-gendered}.
%Moreover, \newcite{cryan:CHI:2020} showed that BERT can be fine-tuned to accurately predict gender orientation of documents.
%These prior studies show that pre-trained contextualised embeddings encode gender-related information.

